Time Will Change Things: An Empirical Study on Dynamic Language Understanding in Social Media Classification

Language features are ever-evolving in the real-world social media environment. Many trained models in natural language understanding (NLU), ineffective in semantic inference for unseen features, might consequently struggle with the deteriorating performance in dynamicity. To address this challenge, we empirically study social media NLU in a dynamic setup, where models are trained on the past data and test on the future. It better reflects the realistic practice compared to the commonly-adopted static setup of random data split. To further analyze model adaption to the dynamicity, we explore the usefulness of leveraging some unlabeled data created after a model is trained. The performance of unsupervised domain adaption baselines based on auto-encoding and pseudo-labeling and a joint framework coupling them both are examined in the experiments. Substantial results on four social media tasks imply the universally negative effects of evolving environments over classification accuracy, while auto-encoding and pseudo-labeling collaboratively show the best robustness in dynamicity.

==> figures/case.tex <==
\begin{figure}[h]\small
    \centering
    \begin{tabular}{|p{7.2cm}|}
    \hline
   \underline{\textbf{Data in $t_{0}$}}    \\
   I've always been \textcolor{blue}{\textit{suspicious}} of \#Dr. Fauci as everything...I mean EVERY THING he said was proven \textcolor{blue}{\textit{wrong}}. Every statement on vaccine...wrong! \#coronavirus\\ 
   %The Deep State \textcolor{blue}{\textit{\#FakeScience}} Establishment led by Fauci cares ZERO about the Immune Health of the Americans. To them every problem is an infectious disease. Every solution is a \#vaccine. Time to DESTROY Big Pharma. \textcolor{blue}{\textit{\#FireFauci}}\\ \\
   Fauci has \textcolor{blue}{\textit{lost all credibility}}. After months of \textcolor{blue}{\textit{bullshit}} he can no longer be trusted. He responds like a \textcolor{blue}{\textit{schill}}. \textcolor{blue}{\textit{\#FireFauci}}\\ 
  \hline
    \hline
      \underline{\textbf{Data in $t_{1}$-$t_{3}$}}    \\
      Sign me up for the first vaccine @realDonaldTrump hates. \textcolor{blue}{\textit{\#IStandWithFauci}}\\ 
      Hey @WhiteHouse \#AnthonyFauci never told anyone on live TV to inject disinfect. That's all. That's the tweet. \#TrumpVirus2020 \#TrumpKillsAmericans \textcolor{blue}{\textit{\#FauciHero}}.\\ 
    \hline
    \hline
    \underline{\textbf{Data in $t_{4}$}}    \\
      Thank you to Dr. Fauci for stepping up to @realDonaldTrump and calling him out on his BULLSHIT. Thank you for being a \textcolor{blue}{\textit{leader}} to those who wanna take COVID-19 serious \textcolor{blue}{\textit{\#ThankYouDrFauci}}\\
    \hline
    \end{tabular}
    %\vspace{-0.5em}
    \caption{Pseudo samples from $t_{0}$, $t_{1}$-$t_{3}$, and $t_{4}$ to show the evolution of public opinion on Fauci in \textsc{Stance-Detection} dataset.}
     % \vspace{-1em}
    \label{caseSentence}
\end{figure}
